Formation of Massive Primordial Stars: Intermittent UV Feedback with Episodic Mass Accretion

We present coupled stellar evolution (SE) and 3D radiation-hydrodynamic (RHD) simulations of the evolution of primordial protostars, their immediate environment, and the dynamic accretion history under the influence of stellar ionizing and dissociating UV feedback. Our coupled SE-RHD calculations result in a wide diversity of final stellar masses covering 10 Msun $\lesssim M_* \lesssim$ 1000 Msun. The formation of very massive ($\gtrsim$ 250 Msun) stars is possible under weak UV feedback, whereas ordinary massive (a few x 10 Msun) stars form when UV feedback can efficiently halt the accretion. This may explain the peculiar abundance pattern of a Galactic metal-poor star recently reported by Aoki et al. (2014), possibly the observational signature of very massive precursor primordial stars. Weak UV feedback occurs in cases of variable accretion, in particular when repeated short accretion bursts temporarily exceed 0.01 Msun/yr, causing the protostar to inflate. In the bloated state, the protostar has low surface temperature and UV feedback is suppressed until the star eventually contracts, on a thermal adjustment timescale, to create an HII region. If the delay time between successive accretion bursts is sufficiently short, the protostar remains bloated for extended periods, initiating at most only short periods of UV feedback. Disk fragmentation does not necessarily reduce the final stellar mass. Quite the contrary, we find that disk fragmentation enhances episodic accretion as many fragments migrate inward and are accreted onto the star, thus allowing continued stellar mass growth under conditions of intermittent UV feedback. This trend becomes more prominent as we improve the resolution of our simulations. We argue that simulations with significantly higher resolution than reported previously are needed to derive accurate gas mass accretion rates onto primordial protostars.

==> table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%                        TABLES                            %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------------------------------------------------------------------%
\begin{table*}[t]
\label{tb:cmd}
\begin{center}
Table 1. Cosmological Cases Considered \\[3mm]
{\scriptsize 
\begin{tabular}{lcccccc}
\hline
\hline
Cases & $N_R \cdot N_\theta \cdot N_\phi$
      & $r_{\rm max}$ ($10^4$~AU) & $M_{\rm g, tot}$ ($\msun$) 
      & $\Delta t$ ($10^4$~yr) & $M_{\rm *, 3D}$ ($\msun$)  
      & $M_{\rm *, 2D}$ ($\msun$) \\
\hline
A     &  $96 \cdot 32 \cdot 64$  & 150 & $1.0 \times 10^4$ & 7
		     & 462.4$^\ast$ & 751.3\\
B     &  $96 \cdot 32 \cdot 64$  & 150 & $1.3 \times 10^4$ & 7
		     & 598.8$^\ast$ & 283.9 \\
B-NF$^\dagger$  &   $96 \cdot 32 \cdot 64$ & 150 &  & 7 & \\
B-NF-HR2$^\ddag$-m0$^\star$ &  $128 \cdot 64 \cdot 128$ & 4 & $1.1
	     \times 10^3$ & 0.3 & \\
B-NF-HR2-m40    &  $128 \cdot 64 \cdot 128$ & 4 & & 0.3 & \\
B-NF-HR2-m70    &  $128 \cdot 64 \cdot 128$ & 4 & & 0.3 & \\
B-NF-HR2-m120   &  $128 \cdot 64 \cdot 128$ & 4 & & 0.3 & \\
B-NF-HR4$^\ddag$-m20  &  $192 \cdot 128 \cdot 256$ & 0.67 & & 0.1 & \\
B-NF-HR4-m20-fc$^\diamond$  & $192 \cdot 128 \cdot 256$ & 0.67 
                            & & 0.1 & \\
B-NF-HR4-m20-lsk$^\bullet$  & $192 \cdot 128 \cdot 256$ & 0.67 
                            & & 0.1 & \\
C     & $64 \cdot 32 \cdot 64$ & 4 & $1.0 \times 10^3$ & 12
      & 286.0 & 160.3 \\
C-HR2-m0      &  $128 \cdot 64 \cdot 128$ & 4 &   & 5.5 & \\ 
D     & $64 \cdot 32 \cdot 64$ & 4 & 490 & 8 & 67.4 & 55.5 \\
D-NF  & $64 \cdot 32 \cdot 64$ & 4 &  & 8 & \\
D-DF$^\dagger$  & $64 \cdot 32 \cdot 64$ & 4 &  & 8 & \\
E     & $96 \cdot 32 \cdot 64$ & 150  & $2.7 \times 10^3$ & 6
		     & 14.3 & 24.4 \\
\hline
\end{tabular}
}
\noindent
\end{center}
Col.\ 2: cell numbers, Col.\ 3: position of the 
radial outer boundary, Col.\ 4: total mass contained in the
 computational domain, Col.\ 5: time duration followed 
Col.\ 6: final stellar masses in the current work,
Col.\ 7: final stellar masses obtained in 2D SE-RHD simulations \citep{Hirano14} 
\\
\\
$^\ast$: Stellar masses at the end of the simulations, 
        $t = 7 \times 10^4$ years. \\ 
$^\dagger$: Suffix ``NF'' represent casess with no UV 
              feedback and ``DF'' with only dissociation (FUV) feedback. \\  
$^\ddag$: Suffix ``HR2'' represents cases with
            doubled and ``HR4'' with quadrupled spatial resolutions. \\
$^\star$: Suffix ``mX'' represents the points for the restart 
            after doubling the resolution when $M_* \simeq {\rm X}~\msun$. \\
$^\diamond$: Stringent limit for the cooling with $f_{\rm limit} = 24$ 
             (see Section~\ref{ssec:flimit}). \\
$^\bullet$: Larger sink cell with $r_{\rm min} \simeq 52$~AU
             ($r_{\rm min} = 30$~AU for all other cases).
\end{table*}
%---------------------------------------------------------------------------------%
%---------------------------------------------------------------------------------%
\begin{table}[t]
\label{tb:chem}
\begin{center}
Table 2. Chemical Reactions Included \\[3mm]
\begin{tabular}{llc}
\hline
\hline
No. & Reactions & References \\
\hline
R1 &  H      +  e  $\rightarrow$ H$^+$ + 2 e        &  1 \\
R2 &  H$^+$  +  e  $\rightarrow$ H     + $\gamma$   &  2 \\
R3$^\dag$ &  H$^-$  +  H  $\rightarrow$ H$_2$ + e   &  3 \\
R4 &  H$_2$  +  H$^+$ $\rightarrow$ H${_2}^+$ + H   &  4 \\
R5 &  H$_2$  +  e     $\rightarrow$ 2 H + e         &  4 \\
R6$^\dag$ &  H$_2$  +  H  $\rightarrow$  3 H        &  5 \\
R7$^\dag$ &  3 H          $\rightarrow$  H$_2$ + H  &  6 \\
R8 &  2 H  + H$_2$ $\rightarrow$  2 H$_2$           &  7 \\
R9 &  2 H$_2$      $\rightarrow$  2 H   + H$_2$     &  7 \\
R10 & H    + e     $\rightarrow$  H$^-$ + $\gamma$  &  4 \\  
R11 & H + $\gamma$ $\rightarrow$  H$^+$ + e         &  2 \\
R12 & H$_2$ + $\gamma$ $\rightarrow$ 2 H            &  8, 9 \\ 
R13 & 2 H          $\rightarrow$  H$^+$ + e + H     &  7 \\ 
R14 & H$^-$ + e    $\rightarrow$  H + 2 e           &  1 \\
R15 & H$^-$ + H$^+$ $\rightarrow$ 2 H               &  4 \\
R16$^*$ & H$^-$ + H$^+$ $\rightarrow$ H$_2^+$ + e       & 4 \\
R17$^*$ & H$^-$ + $\gamma$ $\rightarrow$ H + e          & 10 \\
R18$^*$ & H + H$^+$ $\rightarrow$ H${_2}^+$ + $\gamma$  & 4 \\
R19$^*$ & H${_2}^+$ + H $\rightarrow$ H$_2$ + H$^+$     & 4 \\
R20$^*$ & H${_2}^+$ + e $\rightarrow$ 2 H               & 4 \\
R21$^*$ & H${_2}^+$ + H$^-$ $\rightarrow$ H$_2$ + H     & 11 \\
\hline
\end{tabular}
\noindent
\end{center}
$^\dag$ reaction rates updated with respect to HR14, \\
$^*$ additional reactions added with respect to HR14 \\
\\
REFERENCES: (1) \citealt{Abel97}, (2) \citealt{OF06}, 
(3) \citealt{Kreckel10}, (4) \citealt{GP98}, (5) \citealt{Martin96},
(6) \citealt{Forrey13}, (7) \citealt{PSS83}, (8) \citealt{TH85},
(9) \citealt{DB96}, (10) \citealt{John88}, (11) \citealt{Millar91}
%\tablecomments{}
\end{table}
%------------------------------------------------------------------------------% 


